A Decoupled Spatio-Temporal Framework for Skeleton-based Action Segmentation

Effectively modeling discriminative spatio-temporal information is essential for segmenting activities in long action sequences. However, we observe that existing methods are limited in weak spatio-temporal modeling capability due to two forms of decoupled modeling: (i) cascaded interaction couples spatial and temporal modeling, which over-smooths motion modeling over the long sequence, and (ii) joint-shared temporal modeling adopts shared weights to model each joint, ignoring the distinct motion patterns of different joints. We propose a Decoupled Spatio-Temporal Framework (DeST) to address the above issues. Firstly, we decouple the cascaded spatio-temporal interaction to avoid stacking multiple spatio-temporal blocks, while achieving sufficient spatio-temporal interaction. Specifically, DeST performs once unified spatial modeling and divides the spatial features into different groups of subfeatures, which then adaptively interact with temporal features from different layers. Since the different sub-features contain distinct spatial semantics, the model could learn the optimal interaction pattern at each layer. Meanwhile, inspired by the fact that different joints move at different speeds, we propose joint-decoupled temporal modeling, which employs independent trainable weights to capture distinctive temporal features of each joint. On four large-scale benchmarks of different scenes, DeST significantly outperforms current state-of-the-art methods with less computational complexity.

==> algorithm/algorithm.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[t]  
  \caption{\ourMthd}
  \label{JFormer}  
  \begin{algorithmic}[1]
  \REQUIRE The MoCap skeleton feature $X \in {\mathbb R^{C \times V \times T}}$.
  \ENSURE The category for each frame $P=[p_1, \cdots, p_T]$.
    \STATE $\hat S, H, R \longleftarrow \{\}, \{\}, \{\}.$ 
    \STATE $L_y \longleftarrow$ the number of JTM layers.
    \STATE $L_c = M \longleftarrow$ the number of STI layers.
    \STATE $S = \mbox{Spatial Modeling}(X)$
    \STATE $(\hat S_1, \hat S_2, \cdots, \hat S_i) = \mathcal {R} (\mbox{Divide}(S, M))$
    \FOR{$l=1, \cdots, L_y$}    
      \IF{$l=1$}    
      \STATE $H_{(1)} =\mbox {$\mathcal T$}(\hat S_1)$ 
      \ELSIF{$1< l \leq L_c$}
      \STATE $R_{l-1} =  \mbox {STI}(\hat{S}_{l}, H_{(l-1)})$;\\
      $H_{(l)} =\mbox {$\mathcal T$}(R_{l-1})$ 
      \ELSE
      \STATE $H_{(l)} =\mbox {$\mathcal T$}(H_{(l-1)})$ 
      \ENDIF    
    \ENDFOR 
    \STATE $Y_{c} = {Softmax}(Conv1D (H_{(L_y)}))$
    \STATE $Y_{b} = Sigmoid(Conv1D (H_{(L_y)}))$
    \STATE $Y_{c}^\prime = \mbox {ASB} (Y_{c})$; $Y_{b}^\prime = \mbox {BRB} (Y_{b})$
    % \STATE $Y_{b}^\prime = \mbox {BRB} (Y_{b})$
    \STATE $P \longleftarrow$ Fusing $Y_{c}^\prime $ and $Y_{b}^\prime$
    % \STATE $Y_{c}^\prime = \mbox {ASB} (Y_{c})$
    % \STATE $Y_{b}^\prime = \mbox {BRB} (Y_{b})$
    % \STATE $\mathcal{L} = \mathcal{L}_{\mbox {asb}}() + 0.1 \mathcal{L}_{\mbox {brb}}()$
    \end{algorithmic}
  \end{algorithm}

==> figs/1-Introduction.tex <==
\begin{figure}[t]
  \centering
    \begin{overpic}[width=0.45\textwidth]{images/1-Introduction}
    % (a) Existing Methods
    \put(12,98){\footnotesize{Skeleton Data}}
    \put(23.5,90){\footnotesize{\color{red} Cascaded}}
    \put(23,87){\footnotesize{Interaction}}
    \put(6,92){Spatial}
    \put(4,82.5){Temporal}
    \put(6,70.5){Spatial}
    \put(4,61.5){Temporal}
    \put(36.2,66){\small {Joint-{\color{red} shared} Temporal Modeling}}
    \put(59,76.5){\LARGE $\ast$}
    \put(60,93){\footnotesize{weights}}
    \put(60,88.5){\footnotesize{joint features}}
    \put(45,97.5){\LARGE $\ast$}
    \put(50,98){\footnotesize{convolutional operation}}
    % \put(34,76){$V$}
    % \put(43,68){\footnotesize{$V \times T$}}
    % \put(65.5,72){\footnotesize{$1 \times D$}}
    % \put(39,64){\footnotesize {$V:$ Joint Num  $T:$ Frame Num}} 
    % \put(56.8,60){\footnotesize {$D:$ Kernel Size}} 
    % \put(23.5,68){\footnotesize{Cascaded}}
    % \put(23,65){\footnotesize{Interaction}}
    \put(25,54.5){(a) Existing Methods}
    % (b) DSTF
    \put(8.5,44){Unified Spatial}
    \put(20,50){\footnotesize{Skeleton Data}}
    \put(4,35){Temporal}
    \put(4.5,28.5){\footnotesize{\color{red} Decoupled}}
    \put(4.5,25.5){\footnotesize{Interaction}}
    % \put(8.5,25.8){\Large {$\boldsymbol \otimes$}}
    \put(4,18.5){Temporal}
    \put(4.5,8){\footnotesize{\color{red} Decoupled}}
    \put(4.5,5){\footnotesize{Interaction}}
    % \put(8.5,5.8){\Large {$\boldsymbol \otimes$}}
    \put(59,34.5){\LARGE $\ast$}
    \put(59,29){\LARGE $\ast$}
    \put(59,22.5){\LARGE $\ast$}
    \put(59,17){\LARGE $\ast$}
    \put(34.5,12){\small {Joint-{\color{red} decoupled} Temporal Modeling}}
    \put(6,-3){(b) Decoupled Spatio-Temporal Framework (Ours)}
    \end{overpic}
   \vspace{5pt}
  \caption{Comparison of existing and our proposed methods for spatio-temporal modeling in the skeleton-based action segmentation.
  % 
  (a) Existing methods employ coupled spatial and temporal modeling for \textbf{cascaded} interaction and joint-\textbf{shared} weights for temporal modeling.
  % 
  (b) In contrast, the proposed \ourMthd~\textbf{decouples} the cascaded spatial-temporal interaction and the temporal modeling of different joints, capturing discriminative spatial-temporal representations.
  % As shown in (a) left, existing methods~\cite{filtjens2022skeleton,xu2023efficient,li2023involving} employ the \textbf{cascaded} interaction that adopts coupled spatial and temporal modeling, over-smoothing the spatio-temporal information and introducing high computational costs.
  % 
  % In contrast, \ourMthd~\textbf{decouples} cascaded interaction, which divides spatial features into distinct sub-features that adaptively interact with the temporal features at different layers, respectively.
  % 
  %  
  % (a) Existing methods~\cite{filtjens2022skeleton,xu2023efficient,li2023involving} usually utilize Joint-\textbf{sharing} Temporal Modeling that adopts shared weights across different joints, ignoring the distinctive motion patterns of different joints. 
  % % losing distinctive temporal information.
  % % 
  % Moreover, the \textbf{cascaded} interaction adopts coupled spatial and temporal modeling, over-smoothing the spatio-temporal information and bringing a high computational budget.
  % % Moreover, with the \textbf{cascaded} interaction, 
  % % the multiple coupled Spatial Modeling and JSTM blocks are stacked, resulting in over-smoothing of spatio-temporal information and costing high computational resources.
  % % 
  % (b) In contrast, we propose the Joint-\textbf{wise} Temporal Modeling that models each joint using independent weights, capturing distinctive features from joints.
  % % 
  % \ourMthd~also \textbf{decouples} cascaded interaction, which divides spatial features into distinct sub-features that adaptively interact with the temporal features at different layers, respectively.
  % % 
  % % {$\boldsymbol \otimes$} denotes spatio-temporal interaction,and {$\ast$} represents convolutional operation.
  }
  \label{1-Introduction}
\end{figure}

==> figs/1-RGB-Skeleton.tex <==
\begin{figure}[t]
  \flushright
    \begin{overpic}[width=0.45\textwidth]{images/1-RGB-Skeleton}
    % RGB video-based
    \put(-5,47){\small \emph{RGB video-based}}
    \put(10,39){\small {Camera}}
    \put(40,47.5){\scriptsize {Step1}}
    \put(75,47.5){\scriptsize {Step2}}
    \put(42.5,38){Feature}
    \put(41,34){Extractor}
    \put(70,38){Temporal}
    \put(70,34){Modeling}  
    \put(25,24){\small {Video}}
    \put(48,24){\small {Pre-extracted features}}
    \put(85,24){\small {Prediction}}
    % Skeleton-based
    \put(-5,18){\small \emph{Skeleton-based}}
    \put(10,13){\small {MoCap}}
    \put(50,12){Spatio-temporal}
    \put(55,7){Modeling}  
    \put(15,-3){\small {Skeleton sequence}}
    \put(85,-3){\small {Prediction}}
    \end{overpic}
   \vspace{.2cm}
  \caption{The comparison between the RGB video-based and skeleton-based action segmentation.
  %  
  The RGB video-based TAS is typically performed in two steps: feature extraction and temporal modeling.
  % 
  In contrast, the skeleton-based TAS in this work is conducted in an end-to-end manner with lightweight spatio-temporal modeling.
  }
  \label{RGB-Skeleton}
\end{figure}

==> figs/10-SSM-Class-Short-Middle-Long.tex <==
\begin{figure}[!t]
  \centering
  % \includegraphics[width=0.48\textwidth]{J-STFormer-20231007/images/ssm-score} 
    \begin{overpic}[scale=0.50]{images/10-SSM-Class-Short-Middle-Long}
        % \put(45,0){\scriptsize {Action category}}
        \put(-3,18){\rotatebox{90}{\scriptsize {Acc (\%)}}}
    \end{overpic}
   % \vspace{.1cm}
    % }
  \caption{Effect of SSM at short, middle and long distance on different actions. 
  }
  \label{SSM-Class-Short-Middle-Long}
\end{figure}

==> figs/11-SSM-Scales.tex <==
\begin{figure}[!t]
  \centering

  \begin{overpic}[width=0.48\textwidth]{images/11-SSM-Scales}
    % F1@50
    \put(25,-2){\scriptsize {$K$}}
    \put(-2,15){\rotatebox{90}{\scriptsize {F1@50}}}
    % Acc
    \put(80,-2){\scriptsize {$K$}}
    \put(50,15){\rotatebox{90}{\scriptsize {Acc (\%)}}}
  \end{overpic}
  \vspace{.1cm}
  \caption{Effect of SSM at different scales on MCFS-130 dataset. 
  }
  \label{SSM-Scales}
\end{figure}

==> figs/12-Visualization-STI-Label.tex <==
\begin{figure}[!t]
  \flushright
      \begin{overpic}[width=0.40\textwidth]{images/12-Visualization-STI-Label}
        \put(-20,43){\small {GT}}
        \put(-20,34.5){\small {D}}
        \put(-20,25.5){\small {C}}
        \put(-20,17.5){\small {B}}
        \put(-20,9.5){\small {A}}
        \put(-20,1.5){\small {Baseline}}
    \end{overpic}
   % \vspace{.1cm}
  \caption{The visualization of predictions for various spatio-temporal methods on MCFS-130 dataset. }
  \label{Visualization-STI-Label}
\end{figure}

==> figs/13-Visualization-STI-Tsne.tex <==
\begin{figure}[!t]
  \centering
    \begin{overpic}[width=0.42\textwidth]{images/13-Visualization-STI-Tsne}
        \put(18,-5){Baseline}
        \put(74,-5){D}
    \end{overpic}
   \vspace{.5cm}
  \caption{The feature embeddings of various spatio-temporal methods in a 2D space using t-SNE \cite{van2008visualizing}.
  % 
  The colors indicate the action category of the MCFS-130.
  % 
  The dots represent the last feature embeddings of the encoder that match the ground truth annotations.
  }
  \label{Visualization-STI-Tsne}
\end{figure}

==> figs/2-Comparison-Architecture.tex <==
\begin{figure}[t]
  \centering
    \begin{overpic}[width=0.48\textwidth]{images/2-Comparison-Architecture}
    % (a) MS-TCN
    \put(7,50){\rotatebox{-90} {Temporal}}
    \put(19,50){\rotatebox{-90} {Temporal}}
    \put(34,50){\rotatebox{-90} {Temporal}}
    \put(14,28){{(a) MS-TCN}}
    % (b) MS-GCN
    \put(52,48){\rotatebox{-90} {Spatial}}
    \put(62.5,50){\rotatebox{-90} {Temporal}}
    \put(77,48){\rotatebox{-90} {Spatial}}
    \put(88,50){\rotatebox{-90} {Temporal}}
    \put(60,28){{(b) MS-GCN}}
    % (c) IDT-GCN
    \put(7,20){\rotatebox{-90} {Spatial}}
    \put(19,22){\rotatebox{-90} {Temporal}}
    \put(34,22){\rotatebox{-90} {Temporal}}
    \put(14,1){{(c) IDT-GCN}}
    % (d) 
    \put(52,20){\rotatebox{-90} {Spatial}}
    \put(71,22){\rotatebox{-90} {Temporal}}
    \put(88,22){\rotatebox{-90} {Temporal}}
    \put(60,1){{(d) \ourMthd}}
    \end{overpic}
   % \vspace{.5cm}
  \caption{Existing network architectures vs. \ourMthd~(ours).
  % 
  (a) MS-TCN contains only temporal modeling.
  % 
  (b) MS-GCN alternately stacks spatial and temporal modeling, over-smoothing the spatio-temporal information.
  % 
  (c) IDT-GCN applies a single spatial modeling followed by multiple temporal modeling, resulting in insufficient spatio-temporal interactions. 
  % 
  (d) The proposed \ourMthd~divides spatial features into distinct sub-features that are injected into hierarchical temporal modeling respectively.
  }
  \label{Comparison-Architecture}
\end{figure}


==> figs/3-Framework.tex <==
\begin{figure*}[t]
  \centering
    \begin{overpic}[width=0.9\textwidth]{images/3-Framework} 
    \put(1,2){MoCap Sequence}
    % SSM
    \put(28,20){\footnotesize{$\alpha_{1t}$}}
    \put(24,15){\footnotesize{$\alpha_{2t}$}}
    \put(21,11){\footnotesize{$\alpha_{3t}$}}
    \put(25,6){\footnotesize{$\alpha_{5t}$}}
    \put(34,4){\footnotesize{$\alpha_{4t}$}}
    \put(41,20.5){\rotatebox{-90}{\footnotesize{\textbf{Divide Spatial Features}}}}
    \put(43.5,18){$\hat S_1$}
    \put(43.5,7){$\hat S_2$}
    \put(22,2){\footnotesize{Spatial Modeling}}
    % JTM
    \put(47,20){\footnotesize{$\hat \alpha_{3(t-1)}$}}
    \put(53,20){\footnotesize{$\hat \alpha_{3t}$}}
    \put(56,20){\footnotesize{$\hat \alpha_{3(t+1)}$}}
    \put(47,15){\footnotesize{$\hat \alpha_{4(t-1)}$}}
    \put(53,15){\footnotesize{$\hat \alpha_{4t}$}}
    \put(56,15){\footnotesize{$\hat \alpha_{4(t+1)}$}} 
    \put(47,10){\footnotesize{$\hat \alpha_{5(t-1)}$}}
    \put(53,10){\footnotesize{$\hat \alpha_{5t}$}}
    \put(56,10){\footnotesize{$\hat \alpha_{5(t+1)}$}} 
    \put(62,13){\footnotesize{$H_{(1)}$}} 
    \put(47.5,4){\footnotesize{Joint-wise Temporal}}
    \put(49,2){\footnotesize{Modeling (JTM)}}
    % STI
    \put(69,18){\footnotesize{$H_{(1)}$}} 
    \put(69.5,8){\footnotesize{$\hat S_2$}} 
    \put(69.3,2.5){\footnotesize{Adaptive Interaction}}
    % \put(70,2.5){\footnotesize{Interaction (STI)}}
    \put(85,13){\footnotesize{$R_1$}}
    \put(88.5,11.5){\footnotesize{JTM}} 
    \put(94,1){\footnotesize{$\times L$}}     
    \end{overpic}
   % \vspace{.5cm}
  \caption{Framework of the proposed end-to-end Joint-wise Spatio-temporal Transformer (\ourMthd).
  % 
  The input to \ourMthd~is skeleton sequence ${\mathcal V}$, where ${\alpha_{vt}}$ denotes the feature of the $v$-th joint at frame $t$.
  % 
  We first employ spatial modeling networks to capture spatial features $S$ of the joints.
  % 
  Then the obtained spatial features $S$ are divided into a group of spatial sub-features $\hat S_i \in {\mathbb R^{V \times T}}$ that represent different spatial semantics. 
  % 
  Moreover, JTM module is utilized to model the temporal dependencies of each joint individually, achieving discriminative temporal features $H_{(i)}$. 
  % 
  In the adaptive interaction block, spatial sub-features adaptively interact with temporal features, learning complex spatio-temporal representations $R_i$ from joints.
  }
  \label{Framework}
\end{figure*}

==> figs/5-STI.tex <==
\begin{figure}[t]
  \centering
      \begin{overpic}[width=0.45\textwidth]{images/5-STI}
        % basic interaction
        \put(13,65.5){{Spatial}}
        \put(22,60){$S$}
        \put(16,52){{JTM}}
        \put(22,46){$H_{(1)}$}
        \put(16,34.5){{JTM}}
        \put(22,29){$H_{(2)}$}
        \put(16,12){{JTM}}
        \put(22,7){$H_{(l)}$}
        \put(0,0){{(a) Basic Interaction}}
        % adaptive interaction
        \put(54,65.5){{Spatial Sub-Features}}
        \put(58,59){$\hat S_1$}
        \put(54,54){{JTM}}
        \put(72,59){$\hat S_2$}
        \put(86,59){$\hat S_l$}
        \put(48,48){$H_{(1)}$}
        % \put(50,41){$F, U$}
        % \put(72,51){$Q$}
        \put(61,44){Cross-Attention}     
        \put(67,39){$R_1$}
        \put(62,33){{JTM}}
        \put(56,27){$H_{(2)}$}
        \put(60,20){$H_{(l-1)}$}
        \put(71.5,23.5){Cross-Attention}     
        \put(86,18){$R_{(l-1)}$}
        \put(81,12){{JTM}}
        \put(76,6){$H_{(l)}$}
        \put(50,0){{(b) Adaptive Interaction}}
    \end{overpic}
   \vspace{.2cm}
  \caption{Basic Interaction vs. Adaptive Interaction.
  % 
  (a) Basic Interaction employs single-layer spatial modeling and performs spatio-temporal interaction by simply summing the temporal features of different layers and the same spatial features.
  % 
  (b) Adaptive Interaction injects one of the spatial sub-features into temporal modeling and the remaining spatial sub-features interact with the temporal features via a Cross-Attention scheme.
  % 
  $\oplus$ denotes the elementwise summation, and $l$ is the number of temporal modeling layers.
  }
  \label{STI}
\end{figure}

==> figs/9-Visualization-JTM-JSTM.tex <==

\begin{figure}[!t]
  \centering
    \begin{overpic}[width=0.48\textwidth]{images/9-Visualization-JTM-JSTM}
    % JTM
    \put(1,56){\small {GT}}
    \put(0.5,48){\footnotesize {Pred.}}
    \put(0.5,33){\rotatebox{90} {\footnotesize {Features}}}
    \put(3.5,44){{\scriptsize {1.0}}}
    \put(3.5,39){{\scriptsize {0.5}}}
    \put(3.5,33){{\scriptsize {0.0}}}
    \put(22,32){{\scriptsize {1000}}}
    \put(40,32){{\scriptsize {2000}}}
    \put(57,32){{\scriptsize {3000}}}
    \put(75,32){{\scriptsize {4000}}}
    \put(93,32){{\scriptsize {5000}}}
    \put(96,29){{\scriptsize {T}}}
    \put(25,28.1){\small{(a) Joint-wise Temporal Modeling (ours)}}
    % JSTM
    \put(0.5,22){\footnotesize {Pred.}}
    \put(0.5,9){\rotatebox{90} {\footnotesize {Features}}}
    \put(3.5,17){{\scriptsize {1.0}}}
    \put(3.5,12){{\scriptsize {0.5}}}
    \put(3.5,6){{\scriptsize {0.0}}}
    \put(22,5){{\scriptsize {1000}}}
    \put(40,5){{\scriptsize {2000}}}
    \put(57,5){{\scriptsize {3000}}}
    \put(75,5){{\scriptsize {4000}}}
    \put(93,5){{\scriptsize {5000}}}
    \put(96,1){{\scriptsize {T}}}
    \put(25,1.1){\small {(b) Joint-Sharing Temporal Modeling.}}
    \end{overpic}
   % \vspace{.5cm}
  \caption{The visualization of predictions and temporal features output by JTM and JSTM on a sequence from the MCFS-22 dataset.
  % 
  We present the temporal features of a single channel in the last layer of the models. 
  % 
  Different colors represent different categories of action.
  }
  \label{Visualization-JTM-JSTM}
\end{figure}

==> figs/sub-visualization-mcfs-label.tex <==
\begin{figure*}[t]
  \centering
    \begin{overpic}[width=0.85\textwidth]{images/sub-visualization-mcfs-label}
    % MCFS-130 
    \put(-5,86){GT}
    \put(-5,80){{\ourMthd}}
    \put(-5,75){{IDT-GCN}}
    \put(-5,70){{BCN}}
    \put(-5,65){{ASRF}}
    \put(-5,60){{ETSN}}
    \put(30,48){{(a) n06\_p07 from MCFS-130 dataset.}}
    % MCFS-22
    \put(-5,41){GT}
    \put(-5,35){{\ourMthd}}
    \put(-5,30){{IDT-GCN}}
    \put(-5,25){{ASFormer}}
    \put(-5,20){{BCN}}
    \put(-5,15){{ASRF}}
    \put(-5,10){{ETSN}}
    \put(30,-2){{(b) n30\_p02 from MCFS-22 dataset.}}
    \end{overpic}
   \vspace{.5cm}
  \caption{The visualization of action segmentation on MCFS-130 and MCFS-22 datasets.
  % 
  The different colors represent different action categories.
  }
  \label{sub-visualization-mcfs-label}
\end{figure*}


==> figs/sub-visualization-pku_lara-label.tex <==
\begin{figure*}[t]
  \centering
    \begin{overpic}[width=0.85\textwidth]{images/sub-visualization-pku_lara-label}
    % PKU-MMD (sub)
    \put(0,64){GT}
    \put(0,58){{\ourMthd}}
    \put(0,53){{MS-GCN}}
    \put(0,48){{MS-TCN}}
    \put(1,32){{(a) A01N07-M from PKU-MMD (sub) dataset.}}
    % PKU-MMD (sub)
    \put(52,64){GT}
    \put(52,58){{\ourMthd}}
    \put(52,53){{MS-GCN}}
    \put(52,48){{MS-TCN}}
    \put(53,32){{(b) A06N12-L from PKU-MMD (view) dataset.}}
    % LARA
    \put(0,25){GT}
    \put(0,20){{\ourMthd}}
    \put(0,15){{MS-GCN}}
    \put(0,10){{ASRF}}
    \put(0,5){{MS-TCN}}
    \put(30,-2){{(c) L03\_S07\_R23\_A05\_N01 from LARa dataset.}}
    \end{overpic}
   \vspace{.5cm}
  \caption{The visualization of action segmentation on MCFS-130 and MCFS-22 datasets.
  % 
  The different colors represent different action categories.
  }
  \label{sub-visualization-pku_lara-label}
\end{figure*}


==> tabs/VIII-SSM-Short-Middle-Long.tex <==

\begin{table}[!t]
  \centering
  \setlength{\abovecaptionskip}{0pt}
  \caption{Effect of the spatial modeling with different distances for SSM on MCFS-130 dataset (split \#1).
  % 
  Short, Middle and Long denote the setting of $k \in [1,4]$,  $k \in [5,8]$ and $k \in [9,12]$, respectively.
  }
    \setlength{\tabcolsep}{2.0mm}
    \begin{tabular}{lcccccc}
      \bottomrule
        & F1$@10$ & F1$@25$ & F1$@50$ & Edit & Acc \\
      \midrule
          Short& 74.4 & \textbf{71.2} & \textbf{61.3} & \textbf{74.7} & 69.2 \\
          Middle & 73.4 & 69.3 & 60.9 & 74.1 & 69.6 \\
          Long& \textbf{74.6} & 71.0 & 61.0 & 74.3 & \textbf{70.0} \\
        \toprule 
    \end{tabular}
\label{scale_neighborhood}
\end{table}


==> tabs/XI-SSM-STI-Fine_grained.tex <==
\begin{table}[!t]
  \centering
  \setlength{\abovecaptionskip}{0pt}
  \caption{Comparison of various spatio-temporal methods on fine-grained actions from MCFS-130 dataset (split \#1). 
  We only evaluate fine-grained action segments,~\ie remove the excessive action segments between actions.
  }
\setlength{\tabcolsep}{0.5mm}{
  \begin{tabular}{cccccccc}
  \toprule
  Model&SSF &STI& F1$@10$~$\uparrow$ & F1$@25$~$\uparrow$ & F1$@50$~$\uparrow$ &Edit~$\uparrow$ &Acc~$\uparrow$\\
  \midrule
    \multicolumn{3}{l}{Baseline} & 44.2    & 43.2    & 41.9    & 37.0 & 52.0   \\
     % \multicolumn{3}{c}{Single}   & 44.2    & 43.2    & 41.9    & 37.0 & 52.0   \\
    A&\ding{55} &Sum& 42.4    & 41.8    & 40.6    & 35.4 & 48.7   \\
  B&\ding{52}&Sum & 44.9    & 44.4    & 42.2    & 37.0 & \textbf{53.3}   \\ 
  C&\ding{55} &Cross-attention & 45.6 & 45.1& 43.4 & 37.6 & 53.1 \\
  D&\ding{52}&Cross-attention & \textbf{47.5}& \textbf{47.1}& \textbf{44.9}& \textbf{39.2} & 52.8   \\
  \bottomrule
\end{tabular}}
\label{SSM-STI-Fine_grained}
\end{table}
